A Multi-Store Privacy Measurement of Virtual Reality App Ecosystem

Virtual Reality (VR) has gained increasing traction among various domains in recent years, with major companies such as Meta, Pico, and Microsoft launching their application stores to support third-party developers in releasing their applications (or simply apps). These apps offer rich functionality but inherently collect privacy-sensitive data, such as user biometrics, behaviors, and the surrounding environment. Nevertheless, there is still a lack of domain-specific regulations to govern the data handling of VR apps, resulting in significant variations in their privacy practices among app stores. In this work, we present the first comprehensive multi-store study of privacy practices in the current VR app ecosystem, covering a large-scale dataset involving 6,565 apps collected from five major app stores. We assess both declarative and behavioral privacy practices of VR apps, using a multi-faceted approach based on natural language processing, reverse engineering, and static analysis. Our assessment reveals significant privacy compliance issues across all stores, underscoring the premature status of privacy protection in this rapidly growing ecosystem. For instance, one third of apps fail to declare their use of sensitive data, and 21.5\% of apps neglect to provide valid privacy policies. Our work sheds light on the status quo of privacy protection within the VR app ecosystem for the first time. Our findings should raise an alert to VR app developers and users, and encourage store operators to implement stringent regulations on privacy compliance among VR apps.

==> Chapters/review.tex <==
% \section{Review Analysis}
% can focus privacy concerns from review analysis 

==> Chapters/vr_apk_collection.tex <==
\section{VR app Collection}\label{data_collection}
In this section, we brief the process of VR app details collection (Section~\ref{sec:crawler}) and VR app APK collection (Section~\ref{sec:apk}).
\subsection{Data Collection}\label{sec:crawler}
VR app stores often require app developers to provide meta-information for their apps (shown in Figure~\ref{fig:vr_example}, red meta-information is privacy-related). This privacy-related meta-information includes the app name, age rating, language support, device required, play style, URL of the privacy policy, and so on. 
We follow different strategies to crawl each VR app store. 
For Oculus, Viveport, Microsoft, Steam, and PlayStation, we utilize Selenium~\cite{Selenium} to crawl meta-information about VR apps. Taking Oculus as an example, each page of the app listing contains dozens of apps. We iteratively click the ``Next Page'' button, read the HTML code of each page and save the URLs of the ``details page'' for each app. 
% By accessing these URLs, we obtain all the privacy-related meta-information.

Due to the limited app information provided on the web-based Pico store, we need to obtain meta-information for apps through the mobile version of the Pico store. We deploy multiple Android emulators on a PC and use Appium~\cite{appium2023app} to send commands to simulate clicks on these emulators. Appium packaged the app's textual information into XML format. By parsing the XML files, we could retrieve all the meta-information for each app.


% It is worth noting that the Pico store does not directly provide a link to the privacy policy on the app's properties page instead of a button 
% \paragraph{For Pico:}
% \begin{itemize}
%     \item In regard to the Android version of the Pico Store, it offers data consistent with the in-device store of Pico VR. To expedite the data extraction process, we deployed multiple Android emulators on our PC, operating them concurrently. Using Appium, we dispatched commands to these emulators for various operations, such as swiping and tapping. When an emulator displays the details page of an application, Appium parses the text information on the page into XML format. Common attributes of an app, such as its name and age rating, can be acquired by reading this XML file.
%     \item It is noteworthy that the Pico Store does not directly provide a link to the privacy policy on the application attribute page. However, it offers a button which, when pressed, redirects to a browser displaying the privacy policy. In response, we designed a mock browser to intercept the link being sent to the actual browser from Pico Store.
% \end{itemize}

% \paragraph{For Other Platforms:}
% \begin{itemize}
%     \item For the remaining five platforms, we employed Selenium, a more suitable choice over Beautiful Soup, as it can fully emulate user interactions and thus is less likely to be detected by anti-scraping mechanisms. Given the similarity in data collection across these five platforms, we'll use the Oculus platform as an example. Initially, the platform presents a list of games spanning multiple pages, with each page potentially containing dozens of applications. By continually tapping the "next page" button via Selenium and subsequently reading each page's HTML code, we can garner URLs of detail pages for all applications on that page. For each of these detail pages, we continue with Selenium to retrieve the application's individual attributes. Every successful page visit via Selenium is persisted, meaning its 'page\_source' is saved locally, significantly reducing the time spent on redundant operations.
% \end{itemize}

% \paragraph{Retrieval of the Privacy Policy URLs:}
% \begin{itemize}
%     \item Following steps 1 and 2, we obtained the privacy policy URLs from every platform.
%     \item These URLs generally fall into two categories. The first consists of standard HTML web pages, which can still be accessed using Selenium. The second category includes: 
%     \begin{enumerate}
%         \item URLs ending in .pdf
%         \item Google Docs and other types of online documents. 
%     \end{enumerate}
%     Given the rarity of the second type (\textless{}10 occurrences), our focus remained on the first type. For these, the method involved downloading the .pdf files locally and subsequently reading their content using Python's PDF libraries.
% \end{itemize}

\subsection{APK Collection}\label{sec:apk}
In order to investigate differences between the actual permissions requested by the app and the permissions declared, we need to collect the app's \emph{.apk} files. \emph{.apk} is a file format for Android apps, which contains all the permissions requested by the app in its manifest file. Hence, in this section, we only focus on Android operating system stores (Oculus and Pico).
Unlike traditional mobile apps, VR apps must be downloaded and installed within the virtual environment of VR devices. Therefore, we first create multiple accounts for Oculus and Pico app stores and deploy them on six VR devices. To ensure that we have the latest versions of the apps, we manually download all available apps from both app stores onto the six VR devices. After completing the downloads, we connect the VR devices to a PC and use the ``\emph{pull}'' ADB command to extract the \emph{.apk} of each app installed on the VR devices. In total, we collect \apknum \emph{.apk}, including \oculusapknum from Oculus and \picoapknum from Pico.
% To further explore the correlation between permission requests in VR applications and user privacy, we retrieve APKs from two VR stores: Oculus and Pico.
% The following elucidates the primary reasons and advantages for our choice:
% \subsection{Rationale for Platform Selection}
% \begin{enumerate}
%     \item \textbf{Android-based System Structure:} Both Oculus and Pico utilize an Android-based operating system. Current research on application security and privacy on the Android platform is well-established, with a myriad of tools and methodologies for APK file analysis. This allows us to leverage existing technological foundations for a comprehensive exploration of APKs on these platforms.

%     \item \textbf{Strong Native Application Ecosystem and High User Traffic:} In contrast to Oculus and Pico, many other VR platforms lean more towards PC streaming. Applications in their stores do not form the primary traffic on these platforms. This suggests that APKs from Oculus and Pico are more representative, and their analysis would more accurately reflect real-world user behavior and privacy risks.

%     \item \textbf{Openness and Technical Maturity:} Oculus and Pico both possess significant technological groundwork in the VR industry. These platforms provide developers with a relatively open development environment complemented by a comprehensive set of SDKs and APIs. More importantly, their consistent technological improvements provide our research with a stable benchmark. This stability ensures that our collected data is technically coherent and comparable, thereby enhancing the reliability and accuracy of our research outcomes.
% \end{enumerate}

% \subsection{APK Collection Procedure}
% \paragraph{Obtaining Access Permissions} We initially accessed several accounts that had purchased a vast array of apps on the Oculus and Pico stores. Through these accounts, we could download and install a wide variety of applications, ranging from games to utilities, providing a broad sample for our research.

% \paragraph{Manual Download and Installation} To ensure the most up-to-date version of each application was acquired, reflecting the current state of the store, we opted for manual operations. We individually browsed the Oculus and Pico stores, downloading and installing each application. This manual method, although time-consuming, ensured our data's freshness and reliability.

% \paragraph{Connecting VR Devices to PCs for APK Extraction} After downloading and installing the applications, the next step was to extract them. To do this, a stable connection between the VR device and a PC was essential. We used a USB cable for this connection. Then, ensuring the VR device had developer mode enabled, which allowed us to interact deeply with the device using the ADB tool. Using ADB, a command-line tool for Android device interaction, we could "pull" or copy the APK file from the VR device. Each APK file encapsulated an application, containing its permission requests, resource files, binary codes, etc. Subsequent analysis, such as consistency checks and risky behavior analysis, can then be conducted using these APKs.



